Releasing Large-Scale Human Mobility Histograms with Differential Privacy

Environmental Insights Explorer (EIE) is a Google product that reports aggregate statistics about human mobility, including various methods of transit used by people across roughly 50,000 regions globally. These statistics are used to estimate carbon emissions and provided to policymakers to inform their decisions on transportation policy and infrastructure. Due to the inherent sensitivity of this type of user data, it is crucial that the statistics derived and released from it are computed with appropriate privacy protections. In this work, we use a combination of federated analytics and differential privacy to release these required statistics, while operating under strict error constraints to ensure utility for downstream stakeholders. In this work, we propose a new mechanism that achieves $ \epsilon \approx 2 $-DP while satisfying these strict utility constraints, greatly improving over natural baselines. We believe this mechanism may be of more general interest for the broad class of group-by-sum workloads.

==> pseudocode.tex <==
\begin{algorithm*}[bth]
\caption{Federated DP-FTRL with \colorbox{pink!25}{SecAgg}}
\label{algo:secagg-dp-ftrl}
\begin{algorithmic}
\INPUT: report goal $m$, learning rate for model weights on client $\eta_{c}$ and on server $\eta_{s}$, momentum $\beta=0.9$, noise multiplier for model delta $z_\Delta$,  total number of rounds $T$, \colorbox{pink!25}{fixed clip norm $C$}, and \colorbox{pink!25}{a large scaling parameter $s$}.
\begin{multicols}{2}
\STATE Initialize model $\theta^0$, momentum buffer $\bar{\Delta}^0=0$
\STATE Initialize tree $\tree$ with $z_\Delta$ and $C$
\STATE \colorbox{pink!25}{$d \leftarrow \text{dimension of } \theta^0$}
\STATE \colorbox{pink!25}{$C_\infty \leftarrow \text{ceil} \left(2 s \cdot C \log(d) / \sqrt{d} \right) $}
\STATE \colorbox{pink!25}{$M \leftarrow 2 \cdot C_\infty \cdot m + 1  $ \COMMENT{SecAgg's modulus}}
\STATE \colorbox{pink!25}{$\alpha \leftarrow \exp\left(-0.5\right)  $}
\STATE \colorbox{pink!25}{$\tilde H_{d} \leftarrow \frac{1}{\sqrt{d}} H_{d}$ \COMMENT{Normalized Hadmard matrix}} 

% \STATE $z_\Delta \leftarrow \left( z^{-2} - (2 \sigma_b)^{-2} \right)^{-\sfrac{1}{2}}$
\FOR{each round $t=0, 1, 2, \ldots, T$}
\STATE $\mathcal{Q}^t \leftarrow$ ($m$ users for this round)
\STATE \colorbox{pink!25}{$\xi \leftarrow$ uniform random sign vector $ \in \{-1,+1\}^d$}
\colorbox{pink!25}{\STATE $D_\xi \leftarrow$  diagonal matrix with $\xi$ on the diagonal}

\FOR{each user $i \in \mathcal{Q}^t$ \textbf{in parallel}}
\STATE $\Delta^{t}_i \leftarrow \text{ClientUpdate}(i, \theta^t, \xi)$
\ENDFOR

\STATE \colorbox{pink!25}{\COMMENT{Securely aggregate the model updates}}

 \State  \colorbox{pink!25}{$\Delta_t = \sum_{i \in \mathcal{Q}^k} \Delta^{t}_i \mod{M}$}
  
\STATE \colorbox{pink!25}{\COMMENT{Unshift, unscale, and unrotate}}
 \State  \colorbox{pink!25} {$\Delta_t \leftarrow (1/s) \cdot D_\xi \cdot \tilde{H}_d^T \cdot \left(\Delta_t -C_\infty \right)$}
  
\STATE \COMMENT{Update model weights with noise addition}

\STATE $\tilde{\Delta}^t = \frac{1}{m} \psum \left(\tree, \, {\Delta_t}, \, k \in [0, t] \right)$

\STATE $\bar{\Delta}^t = \beta \bar{\Delta}^{t-1} + \tilde{\Delta}^t$, $\theta^{t+1} \leftarrow \theta^0 + \eta_{s} \bar{\Delta}^t$ 

\ENDFOR
%\ENDFUNCTION

\vspace{1.5ex}
\begin{mdframed}[
    linecolor=black,
    linewidth=1.5pt,
    roundcorner=4pt,
    % backgroundcolor=olive!15,
    userdefinedwidth=1.15\linewidth,
]
\FUNCTION{ClientUpdate($i$, $\theta_0, \xi$)}
\STATE $\theta \leftarrow \theta_0$

\colorbox{pink!25}{\STATE $D_\xi \leftarrow$  diagonal matrix with $\xi$ on the diagonal}
\STATE $\mathcal{G} \leftarrow $ (user $i$'s local data split into batches)
\FOR{batch $g \in \mathcal{G}$}
\STATE $\theta \leftarrow \theta - \eta_c \nabla \ell(\theta;g)$
\ENDFOR
\STATE $\Delta \leftarrow \theta - \theta_0$

\STATE\colorbox{pink!25}{$\Delta \leftarrow \Delta \cdot s \cdot \min{\left(1, \frac{C}{||\Delta||_2}\right)} \quad$  \COMMENT{Scale and $\ell_2$ clip}}

\STATE\colorbox{pink!25}{$\Delta \leftarrow \tilde H_{d} \cdot D_\xi \cdot \Delta$  \COMMENT{Randomly rotate}}

\STATE\colorbox{pink!25}{$\Delta \leftarrow \Delta \cdot \min \left(1, \frac{C_{\infty}}{||\Delta||_{\infty}}  \right)$  \COMMENT{Clip to bound $\ell_\infty$ range}}


\colorbox{pink!25}{ \COMMENT Conditional stochastic rounding}
 \REPEAT
 \STATE $\Delta'\gets$ stochastically round the coordinates of  $\Delta$
  \UNTIL{$\scriptstyle \|\Delta'\|_2^2 \le  s^2C^2 + d/4 + \sqrt{2\log(1/\alpha)} \cdot \left(sC + \sqrt{d} / 2\right)$}
  
\colorbox{pink!25}{\COMMENT Shift to center around $C_\infty$ and apply modulo}
\STATE \colorbox{pink!25}{\textbf{return} $\Delta' + C_\infty  \mod M$}
\ENDFUNCTION
\end{mdframed}
\end{multicols}

\end{algorithmic}
\end{algorithm*}
